Audio Language Model for Deepfake Detection Grounded in Acoustic Chain-of-Thought

Deepfake speech detection systems are often limited to binary classification tasks and struggle to generate interpretable reasoning or provide context-rich explanations for their decisions. These models primarily extract latent embeddings for authenticity detection but fail to leverage structured acoustic evidence such as prosodic, spectral, and physiological attributes in a meaningful manner. This paper introduces CoLMbo-DF, a Feature-Guided Audio Language Model that addresses these limitations by integrating robust deepfake detection with explicit acoustic chain-of-thought reasoning. By injecting structured textual representations of low-level acoustic features directly into the model prompt, our approach grounds the model's reasoning in interpretable evidence and improves detection accuracy. To support this framework, we introduce a novel dataset of audio pairs paired with chain-of-thought annotations. Experiments show that our method, trained on a lightweight open-source language model, significantly outperforms existing audio language model baselines despite its smaller scale, marking a significant advancement in explainable deepfake speech detection.

==> latex/sections/introduction.tex <==
\section{Introduction}

\todo{1.5page is about right, but the first pages looks flat and dull. Add figures?}

\yt{Maybe we can say current multimodal models still rely primarily on large-scale pretraining to align modalities.
However, when faced with distribution shifts (OOD) caused by subtle signal differences, such as artifacts in deepfakes, this implicit alignment is highly fragile.}

Recent advances in text-to-speech (\textbf{TTS}) and voice conversion systems have produced synthetic speech that is increasingly difficult to distinguish from genuine human recordings.
Such \textbf{audio deepfakes} have already been exploited in impersonation attacks, fraud, and misinformation~\citep{bird2023real, yi2023audio, li2025surveydeepfake}, posing serious risks to both individuals and institutions.
As synthesis models continue to evolve, robust and generalizable detection methods have become a central challenge in speech forensics~\citep{todisco2019asvspoof}.

Traditional approaches to audio deepfake detection rely primarily on signal-level artifacts, such as inconsistencies in pitch~\citep{de2012synthetic, pal2018synthetic}, formant trajectories~\citep{sahidullah2015comparison}, energy patterns~\citep{dimitriadis2005auditory}, or voice quality statistics~\citep{javed2022voice}.
While these cues are effective for known generation methods, many detectors suffer from degraded performance under domain shift, particularly when confronted with unseen synthesizers or recording conditions~\citep{kamble2020advances}.
More recent end-to-end neural models~\citep{li2025surveydeepfake, asvspoof2015, asvproof} improve accuracy but largely operate as opaque classifiers, offering limited insight into \textbf{\textit{why}} a given utterance is judged as genuine or synthetic. This lack of interpretability is problematic in high-stakes forensic settings, where human validation and accountability are required.

% Recent progress in advanced text-to-speech models has led to synthetic speech that can deceive both human listeners and automated detectors.
% These synthetic speech impersonating real speakers, called \textit{speech deepfakes} or \textit{audio deepfakes}, have been exploited in scams and impersonation attacks, making reliable detection a critical challenge~\cite{bird2023real, yi2023audio}.


More recently, multimodal large language models (MLLMs) have shown emerging capabilities in reasoning over non-textual inputs, including speech~\citep{baali2025colmbo, yin2025speakerlmendtoendversatilespeaker}.
Existing audio language models can answer questions about audio or perform classification through supervised fine-tuning, but they typically make decisions in a single step, without explicitly articulating how acoustic evidence supports the final judgment. This raises a natural question: \textbf{can explicit, structured reasoning over measurable acoustic attributes improve the reliability, generalization, and transparency of audio deepfake detection?}

\yt{Above paragraphs introduced from this point? Current Audio-LLMs suffer from a \textbf{modality gap}. The core issue is that purely acoustic embeddings (e.g., those produced by WavLM) are high-dimensional and abstract, whereas LLM reasoning operates over discrete, semantically grounded symbols.
If audio embeddings are directly fed into an LLM, the model is effectively guessing rather than performing structured reasoning.
This explains why existing models, even with very large parameter counts, still struggle with fine-grained signal discrimination tasks such as deepfake detection and often show limited robustness.}

% Existing detection systems have relied on certain artifacts found in human speech to identify speech deepfakes. Unlike human speech, synthetic speech typically lacks certain physiological and phonological artifacts, such as breathing rhythms, coarticulation effects, and hesitations. In contrast, synthetic speech often shows over-smoothed formants, irregular pause distributions, or inconsistencies in pitch and energy~\cite{li2025surveydeepfake}. Existing works often use heuritstics or deep learning-based methods to extract audio features and identify deepfakes.~\cite{asvspoof2015, asvproof, li2025surveydeepfake} However, these conventional detection systems are usually limited to domains and are not generalizable. 
% More recently, Multimodal Large Language models (MLLMs) have demonstrated promising capabilities in various tasks, such as speaker identification and profiling, deepfake, etc.~\cite{baali2025colmbo, yin2025speakerlmendtoendversatilespeaker}. With the growing reasoning capabilities of LLMs, an important question arises: whether an explicit, explainable reasoning process can improve MLLMs on specialized tasks such as audio deepfake detection.
% Leveraging LLMs to reason explicitly over structured acoustic evidence offers the potential for both more robust generalization and human-auditable explanations.
% Whereas human speech depicts certain artifacts (breathing rhythm, coarticulation errors, hesitations), deepfakes often exhibit over-smooth formants, atypical pause patterns, or pitch/energy inconsistencies. Traditional detectors encode all features into a single embedding, providing limited interpretability. In contrast, multimodal large language models (LLMs) show promising abilities in tasks such as speaker identification and profiling~\cite{baali2025colmbo, yin2025speakerlmendtoendversatilespeaker}. By utilizing language models to \emph{reason} over structured speech evidence, we aim to deliver more robust decisions and human-auditable explanations.

In this work, we explore this question in the context of paired audio analysis for automatic speaker verification (\textbf{ASV}) and audio deepfake detection (\textbf{ADD}). Given a genuine reference utterance and a query utterance, the model must determine both whether the two recordings originate from the same speaker and whether the query is synthetic. We propose a lightweight audio–language model that combines a pretrained audio encoder with a compact language model through a learned projection module. Crucially, we inject structured acoustic evidence, covering prosodic, spectral, temporal, and voice quality cues, into the language model input and train the model to produce feature-grounded reasoning before emitting its final decision.

To support this reasoning-centric formulation, we curate a new dataset of audio pairs with corresponding chains-of-thought, built from ASVspoof 2019~\cite{asvproof} and VoxCeleb2~\cite{chung2018voxceleb2}, augmented with recent TTS systems. Through supervised reasoning training, our model learns to align acoustic observations with explicit decision rationales, enabling interpretable and comparison-based judgments. Our experiments demonstrate that incorporating feature-guided reasoning improves robustness under synthesizer shift while requiring only a small base language model, pointing toward more transparent and reliable speech forensic systems.

\yt{I think we can propose our work as a neuro-symbolic dual-streaming framework (instead of relying solely on implicit embedding (neurl stream), we also explicitly inject interpretable acoustic features with clear physical meaning (symbolic stream)).
Then, in essence, our method leverages domain knowledge to align implicit perception with explicit reasoning.
}

% In this work, we investigate whether we can exploit the natural language reasoning capabilities of LLMs with audio inputs for the automatic speaker verification \textbf{(ASV)} and audio deepfake detection \textbf{(ADD)} tasks. To that end, we designed a novel and lightweight audio LLM (ALLM) pipeline for the given tasks. Furthermore, we generated a new dataset based on ASVSpoof2019~\cite{asvproof} and VoxCeleb2~\cite{chung2018voxceleb2} to support the reasoning training. 

% 1. We introduce a reasoning-oriented audio–language modeling framework for paired speaker analysis.
% 2. We propose feature-guided chain-of-thought supervision grounded in measurable acoustic cues.
% 3. We construct a new reasoning-aligned dataset for speaker verification and deepfake detection. --> Good Results.

In summary, our key contributions are as follows:
\begin{itemize}[leftmargin=1.2em]
\item \textbf{We propose a novel and lightweight ALLM-based pipeline for ASV and ADD tasks} that integrates audio inputs into LLMs with feature-guided reasoning, surpassing the performance of existing pretrained ALLM on ASVSpoof2019, while using a smaller base model. 
\item \textbf{We curate a new dataset of audio pairs and chain-of-thoughts (CoT) for ASV and ADD} using existing dataset (ASVSpoof2019, VoxCeleb2), state-of-the-art TTS models for new deepfake audio generation, and text-only LLM for CoT generation. 
% Training on the dataset enables us to align our proposed model to the given tasks. 
\item \textbf{We conduct extensive experiments on the tasks} and explore the effectiveness of our proposed method. Our model outperformed pretrained ALLM baseline on the evaluation dataset, and experiment and ablation results show that reasoning process can positively influence the LLM's predictions, demonstrating the effectiveness of our approach. We expect our work to be a step toward a new direction in the development of ALLMs and deepfake detection, and that in the future we can adapt the framework for real-time application. 
\yt{Better data representations outperform larger parameter sizes.}


\end{itemize}



%Given a pair of two short utterances, where the first utterance is a genuine recording of a known speaker, we want to verify 1) whether the second audio belongs to the same speaker, and 2) whether the recording is genuine and not synthesized.
% By finetuning the audio LLM on our own dataset of audio-reasoning pairs, our method is able to outperform existing ALLM checkpoints by a significant amount. 

==> latex/sections/related_work.tex <==
\section{Related Work}
% Self-supervised speech encoders such as wav2vec~2.0~\cite{wav2vec2}, HuBERT~\cite{hubert}, and WavLM~\cite{wavlm} provide transferable audio features.
% Anti-spoofing research has progressed through the ASVspoof challenges~\cite{asvproof} and dedicated architectures such as AASIST~\cite{aasist}.
% More recently, audio-capable large language models (LLMs), including Whisper-based pipelines~\cite{radford2023robust}, SALMONN~\cite{salmonn}, Qwen-Audio~\cite{qwenaudio}, and WavLLM~\cite{hu20wavllm}, have demonstrated emerging abilities in speech reasoning and instruction following.
% In parallel, chain-of-thought prompting has been shown to enhance reasoning in text-based LLMs~\cite{cot}, yet its application to speech deepfake detection remains largely unexplored.
% Our work bridges these directions by coupling structured acoustic evidence with LLM reasoning to distinguish authentic speech from synthetic mimicry.

\todo{not well written, may want to rework, split to more sections, and truncate. Ref ALLM4ADD}

\paragraph{Audio deepfake detection}
In the past few years, driven by the creation of new datasets and public challenges like ASVspoof~\cite{ asvproof, Todisco2019ASVspoof2019, Wang2024ASVspoof5, FoR2019FakeOrReal}, the field of audio deepfake detection has seen significant progress. While traditional approaches use existing acoustic feature extraction methods for classification, which are explainable but suffer from poorer performance, recent methods have overwhelmingly relied on deep learning. These methods can be categorized into two architectures: (a) separate audio feature extraction and classification, and (b) end-to-end detection~\cite{kamble2020advances, li2025surveydeepfake}. 

In the first type of architecture, a feature extractor (either heuristic or learned) is combined with a classification model to predict the speech authenticity. The two-stage architecture is more popular than the end-to-end architecture due to less training required: for example, pretrained encoders like wav2vec 2.0 or HuBERT~\cite{wav2vec2, hubert} can be used by audio deepfake detection models as the feature extractor~\cite{xie2023learning, lu2024one, wang2024can}. For classification, CNN, LCNN or Transformer-based architectures are often used and trained from scratch for the task~\cite{tomilov2021stc, lavrentyeva2019stc}.
However, this approach separates the extractors and classifier, leading to some loss of information. Moreover, the pretrained extractors are trained on objectives unrelated to deepfake detection, and thus may not sufficiently represent information needed for the task~\cite{wavlm, hu20wavllm}.

In contrast, end-to-end architecture takes waveforms or spectrograms as inputs to directly predict if the utterance in question is real or fake. \cite{teng2022sasasv} proposes a fully trainable end-to-end system that integrates a waveform encoder with multiple classifiers and a pretrained automatic speaker verification system into one trainable model. \cite{mun2023towards} proposes a multi-stage framework that trains the model to learn both ASV and deepfake detection simultaneously. While end-to-end architecture shows promising results, the impact of increased computation costs remain to be discussed.

\paragraph{Large language models for audio tasks}
In recent years, multimodal large language models (MLLMs) have been widely studied and applied to various audio-related tasks. Audio LLMs, including Whisper-based pipelines~\cite{radford2023robust}, SALMONN~\cite{salmonn}, Qwen-Audio~\cite{qwenaudio}, and WavLLM~\cite{hu20wavllm}, have demonstrated emerging abilities in speech reasoning and instruction following in tasks such as speech recognition and audio captioning.

Recent works have focused on adapting LLMs to specific downstream audio tasks outside of ALLM's conventional training data. For example, Cheng et al.~\cite{cheng2024emotion} feeds LLMs with video and audio of humans to predict their emotion. CoLMBo~\cite{baali2025colmbo} proposed embedding the speaker's characteristics into the LLM context, enhancing the performance on tasks like speaker profiling and speaker recognition. 
In the field of deepfake speech detection, ALLM4ADD \cite{allm4add} is the first work utilizing audio LLMs to study the problem, reformulating audio deepfake detection as an audio question answering problem, and further performed supervised fine-tuning on the task with LoRA~\cite{lora}. However, ALLM4ADD still relied on Whisper as its sole audio encoder, which limits the method's interpretability. %In contrast, our proposed method utilizes both the pretrained audio encoder and other feature extractors, ...


